A Stochastic Record-Value Approach to Global Simulation Optimization

Black-box optimization is ubiquitous in machine learning, operations research and engineering simulation. Black-box optimization algorithms typically do not assume structural information about the objective function and thus must make use of stochastic information to achieve statistical convergence to a globally optimal solution. One such class of methods is multi-start algorithms which use a probabilistic criteria to: determine when to stop a single run of an iterative optimization algorithm, also called an inner search, when to perform a restart, or outer search, and when to terminate the entire algorithm. Zabinsky, Bulger & Khompatraporn introduced a record-value theoretic multi-start framework called Dynamic Multi-start Sequential Search (DMSS). We observe that DMSS performs poorly when the inner search method is a deterministic gradient-based search. In this thesis, we present an algorithmic modification to DMSS and empirically show that the Revised DMSS (RDMSS) algorithm can outperform DMSS in gradient-based settings for a broad class of objective test functions. We give a theoretical analysis of a stochastic process that was constructed specifically as an inner search stopping criteria within RDMSS. We discuss computational considerations of the RDMSS algorithm. Finally, we present numerical results to determine its effectiveness.

==> CHANGES <==

March 3, 2015

Renamed my \singlespace to \uwsinglespace to avoid collision with setspace style.



